EVSO: Environment-aware Video Streaming Optimization of Power Consumption

Streaming services gradually support high-quality videos for better user experience. However, streaming high-quality video on mobile devices consumes a considerable amount of energy. This paper presents the design and prototype of EVSO, which achieves power saving by applying adaptive frame rates to parts of videos with a little degradation of the user experience. EVSO utilizes a novel perceptual similarity measurement method based on human visual perception specialized for a video encoder. We also extend the media presentation description, in which the video content is selected based only on the network bandwidth, to allow for additional consideration of the user's battery status. EVSO's streaming server preprocesses the video into several processed videos according to the similarity intensity of each part of the video and then provides the client with the processed video suitable for the network bandwidth and the battery status of the client's mobile device. The EVSO system was implemented on the commonly used H.264/AVC encoder. We conduct various experiments and a user study with nine videos. Our experimental results show that EVSO effectively reduces energy consumption when mobile devices use streaming services by 22% on average and up to 27% while maintaining the quality of the user experience.

==> sections/discussion_and_future_work.tex <==
% 0.5 page

%뉘앙스가 내 한계는 알고있다!
%Discussion and future work은 디테일하게 쓰지마, 걍 문제를 알고있다!

%\section{Efficient EVSO Deployment Methodology}\label{sec:efficient}

% 모든 video를 scheduling 하지 않기!
% Logging 긱법
% selective video processing
% MEC에의 적용
%--

% 우리는 플랜하고 있다. 더 power consumption을 향상하면서 user experience 영향을 최소화할 수 있는지

%실험의 비디오 갯수가 적다. 타입도 늘리고 해야겠다

% 핸드폰이 최신버전이 아님
